Beyond Static Bias: Adaptive Multi-Fidelity Bandits with Improving Proxies

As an extension of the classical multi-armed bandit problem, multi-fidelity multi-armed bandits (MF-MAB) enable individual arms to be evaluated using diverse feedback sources that vary in both cost and accuracy. Prior stochastic models typically assume fixed low-to-high fidelity discrepancies, whereas modern proxy sources, such as learning-based simulators and Large Language Models (LLMs), can be improved using additional calibration. We investigate adaptive MF-MAB with improving proxy sources, and focus on the canonical two-fidelity case in which the low-fidelity source becomes more informative with repeated use. To capture this dynamic, we introduce a selected-average mismatch bound that converts dynamic low-fidelity observations into improvement-aware confidence bounds for the high-fidelity target. We propose the Threshold-Based Adaptive Continuation Companion (TACC), an optimistic algorithm that uses a bounded continuation rule to decide when low-fidelity sampling remains cost-effective and when to escalate. We prove an instance-dependent regret bound showing that, for detected intermediate arms, adaptive continuation replaces logarithmic high-fidelity confirmation with bounded low-fidelity continuation. Experiments on synthetic bandits and an LLM-as-a-judge policy-evaluation task examine when continuation improves cost-weighted regret.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We claim the contributions and scope in abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of assumption in the discussion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For the main theoretical result we provide full set of assumptions and proof in both main context and appendix
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:\answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The details of both synthetic simulation and LLM experiment are disclosed in Experiments section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will package the code of our experiments and submit. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provide the details of experimental setting such as bandit environment generation and parameter chosen.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper reports error bars for all experimental results. These error bars represent the standard deviation calculated across independent trials with different random seeds.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All simulations and LLM-policy experiments are conducted on a local device.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Upon review, we verify that the research conform with the NeurIPS Code of Ethics
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper contribute to an adaptive method to a new bandit problem setting, it does not impact society at large. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experiments are based on synthetic simulations and LLM-policy experiments, which do not include the release of pre-trained models or datasets scraped from the Internet. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite the reference paper and models in our paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will release our code along with detailed README files. The release does not include source code copied from external libraries; all code provided is our own.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research presented is based entirely on synthetic simulations and LLM-policy experiments, and it does not involve human subjects or sensitive user data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research presented is based entirely on synthetic simulations and LLM-policy experiments, and it does not involve human subjects or sensitive user data. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the LLM-policy experiment, we describe the generation and usage of LLM-as-weak-judge model.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/01_intro.tex <==
\section{Introduction}

Multi-fidelity bandits model decision making under heterogeneous information sources: a learner may query a cheap but inaccurate source or a more expensive and more reliable one. Classical formulations assume that the discrepancy between fidelities is fixed or uniformly bounded in advance \citep{kandasamy2016multi,wang2023revisited}. In many modern applications, however, the cheap source is itself adaptive or improvable. A large language model used as a weak judge, a simulator refined by repeated calibration, or a progressively tuned heuristic scorer may become more accurate as it is queried more often.

This paper studies a stylized stochastic bandit model for this phenomenon. We consider two fidelities: a high-fidelity source that defines the target means, and a low-fidelity source whose bias shrinks with the number of low-fidelity queries of the corresponding arm. The main challenge is that fidelity choice is no longer static. At coarse levels of precision, low fidelity may be overwhelmingly cost effective. At finer resolutions, high fidelity may become preferable once the residual low-fidelity bias becomes the dominant source of uncertainty.

Our starting point is a simple but important modeling choice: low-fidelity empirical means should not be interpreted as estimating an instantaneous low-fidelity mean. Instead, they estimate a selected-average quantity indexed by the number of low-fidelity queries. This lets us combine concentration with a shrinking bias envelope in a clean way. Building on this view, we turn fidelity choice into a resolution-dependent decision problem. For each arm and each target precision scale $\eps$, we define the minimum cost needed to shrink uncertainty to scale $\eps$ using either fidelity. This produces an oracle complexity quantity $c_k^\star(\eps;\Lambda)$ that summarizes the cost of information acquisition in the presence of self-improving low fidelity.

We then analyze a phase-based elimination algorithm. At phase $r$, the algorithm targets resolution $\eps_r = 2^{-r}$, chooses for each active arm the fidelity that can reach that resolution at minimum cost, and eliminates arms whose confidence intervals are separated. This perspective naturally replaces earlier case-based reasoning about ``which fidelity is better'' with a single resolution-dependent principle.

Our current technical contribution is an oracle-envelope benchmark. Under a shrinking-bias model and sub-Gaussian noise, we prove an oracle regret bound of the form
\[
R(\Lambda)
\lesssim
\sum_{k\neq k^\star} \Delta_k c_k^\star(\Delta_k/4;\Lambda)
+ \text{lower-order terms},
\]
followed by a generic gap-independent corollary obtained by truncation. This benchmark clarifies the structure of self-improving multi-fidelity problems and provides a foundation for future adaptive model-selection extensions.

\paragraph{Contributions.}
Our current progress can be summarized as follows.
\begin{enumerate}[leftmargin=1.5em]
    \item We formalize a self-improving two-fidelity stochastic bandit model in which the low-fidelity bias shrinks with the number of low-fidelity queries.
    \item We introduce a selected-average interpretation of low-fidelity empirical means and derive valid target confidence intervals by combining concentration with a shrinking bias envelope.
    \item We formulate fidelity choice as a resolution-dependent decision problem and define the oracle complexity quantity $c_k^\star(\eps;\Lambda)$.
    \item We propose a phase-based elimination algorithm and prove an oracle regret theorem together with a generic gap-independent corollary.
\end{enumerate}

\paragraph{Scope.}
The present draft focuses on the clean oracle-envelope version of the theory. We do not yet claim a fully adaptive model-selection result in the main text. Rather, we isolate the benchmark that an adaptive extension should compete with.


==> sections/02_related_work.tex <==
\section{Related Work}

\paragraph{Multi-fidelity bandits.}
The multi-fidelity bandit model was introduced by \citet{kandasamy2016multi}, who considered stochastic bandits with multiple fidelities and fixed fidelity-specific approximation errors. Their algorithm, MF-UCB, balances statistical uncertainty and static fidelity bias through a fidelity escalation rule. More recently, \citet{wang2023revisited} revisited multi-fidelity multi-armed bandits for both best-arm identification and regret minimization, and \citet{poiani2024optimal} developed an asymptotically optimal approach for multi-fidelity best-arm identification. In all of these works, the fidelity discrepancy is treated as static. Our setting differs in that the low-fidelity source improves with usage, so the preferred fidelity becomes resolution dependent.

\paragraph{Gap-dependent and gap-independent analyses.}
Our regret analysis follows the standard distinction between instance-dependent and distribution-free bounds from the stochastic bandit literature \citep{lattimore2020bandit,bubeck2012regret}. The gap-dependent term in our main theorem is arm specific and fidelity aware through the cost complexity $c_k^\star(\eps;\Lambda)$. The gap-independent corollary is obtained by a truncation argument analogous in spirit to classical conversions from instance-dependent to distribution-free guarantees.

\paragraph{Phase elimination and confidence-based exploration.}
The use of dyadic resolutions and elimination steps is closely related to classical confidence-based pure exploration and regret minimization methods. What is new here is that the elimination schedule is coupled with a resolution-dependent fidelity choice: each active arm is queried at whichever fidelity can most cheaply drive its uncertainty below the current target scale.

\paragraph{Model selection perspective.}
The quantity $c_k^\star(\eps;\Lambda)$ also connects our framework to online model selection. At each target resolution $\eps$, the learner effectively chooses between candidate information sources. In the present draft we analyze an oracle benchmark in which the shrinking bias envelopes are known. A natural next step is to replace this oracle decision rule by a master procedure over candidate surrogate classes, in the spirit of online model selection for bandits \citep{pacchiano2020model}.


==> sections/04_method.tex <==
\section{Method: Resolution-Dependent Fidelity Elimination}
\label{sec:method}

Under improving low fidelity, fidelity choice should not be treated as a static arm-dependent decision. Instead, it should depend on the \emph{target resolution} at which the learner is trying to certify suboptimality. This leads to a clean oracle benchmark: at each scale $\varepsilon$, we ask which fidelity can reduce uncertainty to that scale at lower cost. The resulting phase-based elimination algorithm is the natural benchmark induced by the oracle-envelope model of Section~\ref{sec:problem}.

For the budget horizon $\Lambda$, we use the budget-uniform confidence radius
\begin{equation}
G_\Lambda(n,\delta)
:=
\sqrt{
\frac{\rho \log(4KT_\Lambda^2/\delta)}{n}
},
\qquad n\ge 1,
\end{equation}
where $\rho>0$ is a problem-dependent constant.

Let $N_{k,t}^{(L)}$ and $N_{k,t}^{(H)}$ denote the numbers of low- and high-fidelity queries of arm $k$ before round $t$, and let $\hat{\mu}_{k,t}^{(L)}$ and $\hat{\mu}_{k,t}^{(H)}$ denote the corresponding empirical means. The low-fidelity confidence radius is
\[
\operatorname{rad}_{k}^{(L)}(n,\delta)
:=
G_\Lambda(n,\delta)+B_k(n),
\]
while the high-fidelity confidence radius is
\[
\operatorname{rad}^{(H)}(n,\delta)
:=
G_\Lambda(n,\delta).
\]
The corresponding confidence bounds for the shared target mean $\mu_k^{(H)}$ are
\[
\mathrm{UCB}_{k,t}^{(L)}
=
\hat{\mu}_{k,t}^{(L)}+\operatorname{rad}_{k}^{(L)}(N_{k,t}^{(L)},\delta),
\qquad
\mathrm{LCB}_{k,t}^{(L)}
=
\hat{\mu}_{k,t}^{(L)}-\operatorname{rad}_{k}^{(L)}(N_{k,t}^{(L)},\delta),
\]
and
\[
\mathrm{UCB}_{k,t}^{(H)}
=
\hat{\mu}_{k,t}^{(H)}+\operatorname{rad}^{(H)}(N_{k,t}^{(H)},\delta),
\qquad
\mathrm{LCB}_{k,t}^{(H)}
=
\hat{\mu}_{k,t}^{(H)}-\operatorname{rad}^{(H)}(N_{k,t}^{(H)},\delta).
\]
Thus both fidelities yield valid intervals for the same target quantity $\mu_k^{(H)}$, but with different cost--accuracy trade-offs: low fidelity carries the extra plug-in bias term $B_k(n)$, whereas high fidelity does not.

\begin{lemma}[Valid confidence intervals]
\label{lem:ci}
Fix a budget $\Lambda>0$ and let $T_\Lambda=\lceil \Lambda/\lambda^{(L)}\rceil$. Under Assumptions~\ref{ass:noise} and \ref{ass:plugin}, there exists an event $\mathcal{E}_\Lambda$ with probability at least $1-\delta$ such that on $\mathcal{E}_\Lambda$, for all arms $k\in[K]$ and all rounds $t\le T_\Lambda$,
\begin{equation}
\mu_k^{(H)} \in \bigl[\mathrm{LCB}_{k,t}^{(L)},\,\mathrm{UCB}_{k,t}^{(L)}\bigr]
\quad\text{and}\quad
\mu_k^{(H)} \in \bigl[\mathrm{LCB}_{k,t}^{(H)},\,\mathrm{UCB}_{k,t}^{(H)}\bigr].
\end{equation}
\end{lemma}

We defer the proof to Appendix~\ref{app:proofs}. The key point is that low-fidelity empirical means concentrate around the selected-average quantity $\bar{\mu}_k^{(L)}(n)$, while $B_k(n)$ controls the mismatch between $\bar{\mu}_k^{(L)}(n)$ and the target mean $\mu_k^{(H)}$.

We now formalize fidelity choice at a prescribed resolution level $\varepsilon>0$. The low-fidelity certification cost for arm $k$ is
\[
\mathsf{c}_{k}^{(L)}(\varepsilon;\Lambda)
:=
\lambda^{(L)}
\min\Bigl\{
n\ge 1:
G_\Lambda(n,\delta)+B_k(n)\le \varepsilon/8
\Bigr\},
\]
and the high-fidelity certification cost is
\[
\mathsf{c}^{(H)}(\varepsilon;\Lambda)
:=
\lambda^{(H)}
\min\Bigl\{
n\ge 1:
G_\Lambda(n,\delta)\le \varepsilon/8
\Bigr\}.
\]
With the convention that the minimum of an empty set is $+\infty$, define the oracle cost complexity
\begin{equation}
\mathsf{c}_k^\star(\varepsilon;\Lambda)
:=
\min\bigl\{
\mathsf{c}_{k}^{(L)}(\varepsilon;\Lambda),\,
\mathsf{c}^{(H)}(\varepsilon;\Lambda)
\bigr\},
\end{equation}
and the associated oracle fidelity choice
\[
m_k^\star(\varepsilon;\Lambda)
\in
\operatorname*{arg\,min}
\bigl\{
\mathsf{c}_{k}^{(L)}(\varepsilon;\Lambda),\,
\mathsf{c}^{(H)}(\varepsilon;\Lambda)
\bigr\}.
\]
This makes the role of improvement explicit: at coarse resolutions, low fidelity may be cheaper because its statistical uncertainty shrinks quickly and the residual bias is still tolerable; at finer resolutions, high fidelity may become preferable once the bias term $B_k(n)$ dominates the remaining uncertainty.

This resolution view naturally leads to a phase-based elimination scheme. Let
\begin{equation}
\varepsilon_r := 2^{-r},
\qquad r=1,2,\dots,
\end{equation}
and interpret phase $r$ as targeting resolution $\varepsilon_r$. In that phase, each surviving arm is queried at the cheaper fidelity for reaching scale $\varepsilon_r/8$. Once this is done, every surviving arm has a confidence interval of width at most $\varepsilon_r/4$, so any arm whose gap exceeds $\varepsilon_r$ can no longer remain competitive. This is the basic reason for the phase-elimination design.

We initialize the active set as $\mathcal{S}_1=[K]$. At phase $r$, each surviving arm $k\in\mathcal{S}_r$ is queried at fidelity $m_k^\star(\varepsilon_r;\Lambda)$ until its confidence radius drops below $\varepsilon_r/8$. We then form a confidence interval $[\mathrm{LCB}_{k,r},\mathrm{UCB}_{k,r}]$ of width at most $\varepsilon_r/4$, choose
\[
\hat{k}_r \in \operatorname*{arg\,max}_{k\in\mathcal{S}_r}\mathrm{LCB}_{k,r},
\]
and eliminate every arm whose upper confidence bound is below $\mathrm{LCB}_{\hat{k}_r,r}-\varepsilon_r/4$. The active set is updated as
\begin{equation}
\mathcal{S}_{r+1}
:=
\bigl\{
k\in\mathcal{S}_r:\,
\mathrm{UCB}_{k,r}\ge \mathrm{LCB}_{\hat{k}_r,r}-\varepsilon_r/4
\bigr\}.
\end{equation}

For simplicity, the algorithm uses a constant-cost warm start of one query per arm per fidelity. This adds only an $O(K(\lambda^{(L)}+\lambda^{(H)}))$ lower-order term and avoids defining confidence radii at zero samples.

\begin{algorithm}[t]
\caption{Resolution-Dependent Fidelity Elimination (RDFE)}
\label{alg:rdfe}
\begin{algorithmic}[1]
\Require number of arms $K$, costs $(\lambda^{(L)},\lambda^{(H)})$, confidence level $\delta$, budget $\Lambda$
\State for each arm $k\in[K]$, query once at low fidelity and once at high fidelity
\State initialize all empirical means and counts from the warm start
\State $\Lambda_{\mathrm{used}}\gets K(\lambda^{(L)}+\lambda^{(H)})$, $r\gets 1$, $\mathcal{S}_1\gets [K]$
\While{$\Lambda_{\mathrm{used}} \le \Lambda$ and $|\mathcal{S}_r|>1$}
    \State $\varepsilon_r \gets 2^{-r}$
    \State $\mathrm{completed}\gets \textsc{True}$
    \For{each arm $k\in\mathcal{S}_r$}
        \State choose
        \[
        m_{k,r}\in \operatorname*{arg\,min}
        \bigl\{
        \mathsf{c}_{k}^{(L)}(\varepsilon_r;\Lambda),\,
        \mathsf{c}^{(H)}(\varepsilon_r;\Lambda)
        \bigr\}
        \]
        \If{$m_{k,r}=L$}
            \While{$G_\Lambda(N_k^{(L)},\delta)+B_k(N_k^{(L)}) > \varepsilon_r/8$}
                \If{$\Lambda_{\mathrm{used}}+\lambda^{(L)}>\Lambda$}
                    \State $\mathrm{completed}\gets \textsc{False}$
                    \State \textbf{break}
                \EndIf
                \State query arm $k$ at low fidelity
                \State update $\hat{\mu}_k^{(L)}$, $N_k^{(L)}$, and $\Lambda_{\mathrm{used}}\gets \Lambda_{\mathrm{used}}+\lambda^{(L)}$
            \EndWhile
            \If{$\mathrm{completed}=\textsc{False}$}
                \State \textbf{break}
            \EndIf
            \State set
            \[
            \mathrm{UCB}_{k,r}\gets
            \hat{\mu}_k^{(L)} + G_\Lambda(N_k^{(L)},\delta)+B_k(N_k^{(L)}),
            \qquad
            \mathrm{LCB}_{k,r}\gets
            \hat{\mu}_k^{(L)} - G_\Lambda(N_k^{(L)},\delta)-B_k(N_k^{(L)})
            \]
        \Else
            \While{$G_\Lambda(N_k^{(H)},\delta) > \varepsilon_r/8$}
                \If{$\Lambda_{\mathrm{used}}+\lambda^{(H)}>\Lambda$}
                    \State $\mathrm{completed}\gets \textsc{False}$
                    \State \textbf{break}
                \EndIf
                \State query arm $k$ at high fidelity
                \State update $\hat{\mu}_k^{(H)}$, $N_k^{(H)}$, and $\Lambda_{\mathrm{used}}\gets \Lambda_{\mathrm{used}}+\lambda^{(H)}$
            \EndWhile
            \If{$\mathrm{completed}=\textsc{False}$}
                \State \textbf{break}
            \EndIf
            \State set
            \[
            \mathrm{UCB}_{k,r}\gets
            \hat{\mu}_k^{(H)} + G_\Lambda(N_k^{(H)},\delta),
            \qquad
            \mathrm{LCB}_{k,r}\gets
            \hat{\mu}_k^{(H)} - G_\Lambda(N_k^{(H)},\delta)
            \]
        \EndIf
    \EndFor
    \If{$\mathrm{completed}=\textsc{False}$}
        \State \textbf{break}
    \EndIf
    \State choose
    \[
    \hat{k}_r \in \operatorname*{arg\,max}_{k\in\mathcal{S}_r} \mathrm{LCB}_{k,r}
    \]
    \State update the active set by
    \[
    \mathcal{S}_{r+1}
    \gets
    \bigl\{
    k\in\mathcal{S}_r:\,
    \mathrm{UCB}_{k,r}\ge \mathrm{LCB}_{\hat{k}_r,r}-\varepsilon_r/4
    \bigr\}
    \]
    \State $r\gets r+1$
\EndWhile
\State \Return any arm in the final active set
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:rdfe} is the benchmark policy induced by the oracle-envelope model of Section~\ref{sec:problem}. The contribution is therefore not that arbitrary improving low-fidelity processes can always be handled adaptively without structural information, but rather that once a valid selected-average bias certificate is available, there is a clean resolution-dependent fidelity rule whose regret can be characterized explicitly.

\begin{remark}
\label{rem:why-rdfe}
RDFE is used in the main text for three reasons. First, it is the direct algorithmic realization of the benchmark quantity $\mathsf{c}_k^\star(\varepsilon;\Lambda)$, so the algorithm, proof strategy, and main theorem are organized around the same object. Second, the phase schedule makes the paper’s central message fully explicit: under shrinking fidelity gaps, fidelity choice is a certification problem at scale $\varepsilon$, not a fixed arm-dependent rule. Third, RDFE yields the cleanest closed theorem stack in the current draft, from confidence validity to phase elimination and regret. For this reason, more online or more general variants are deferred to the appendix.
\end{remark}

% Appendix~\ref{app:proofs} records two complementary variants. The first is an online continuation-style surrogate that is more myopic and round-by-round, but it introduces extra continuation-specific mechanisms and parameters and is therefore less cleanly aligned with the oracle quantity $\mathsf{c}_k^\star(\varepsilon;\Lambda)$. The second is a more general dynamic-good-fidelity LUCB primitive for the broader multi-fidelity setting, but in the current draft it mainly serves as a proof roadmap rather than a fully closed main-text theorem stack. These variants are useful for intuition and future extensions, but RDFE remains the clearest main-text algorithm for the present oracle-envelope benchmark.

==> sections/05_theory.tex <==
\section{Theory}
\label{sec:theory}

The analysis proceeds in three steps. We first record the phase-end confidence-width guarantee implied by Algorithm~\ref{alg:rdfe}. We then show that once the target resolution falls below the suboptimality gap of an arm, that arm cannot survive the current phase. Finally, we convert this phase-wise elimination guarantee into a regret bound through the oracle cost complexity $\mathsf{c}_k^\star(\cdot;\Lambda)$.

For bookkeeping, call a phase $r$ \emph{completed} if the algorithm finishes processing every arm in $\mathcal{S}_r$ and performs the elimination update that defines $\mathcal{S}_{r+1}$. Let $R_\Lambda$ denote the number of completed phases under budget $\Lambda$. For a completed phase $r\le R_\Lambda$ and an arm $k\in\mathcal{S}_r$, let
\begin{equation}
\Delta\Lambda_{k,r}
\end{equation}
denote the additional cost spent on arm $k$ during phase $r$. If $k\notin\mathcal{S}_r$, we set $\Delta\Lambda_{k,r}:=0$.

\begin{lemma}[Phase-end confidence width]
\label{lem:phase-width}
Fix a budget $\Lambda>0$ and suppose that the event $\mathcal{E}_\Lambda$ in Lemma~\ref{lem:ci} holds. If phase $r$ is completed, then for every arm $k\in\mathcal{S}_r$,
\begin{equation}
\mu_k^{(H)}\in[\mathrm{LCB}_{k,r},\mathrm{UCB}_{k,r}]
\qquad\text{and}\qquad
\mathrm{UCB}_{k,r}-\mathrm{LCB}_{k,r}\le \varepsilon_r/4.
\end{equation}
\end{lemma}

\begin{proof}[Proof sketch]
By construction, phase $r$ queries each active arm until its relevant confidence radius is at most $\varepsilon_r/8$. If the chosen fidelity is low, then
\begin{equation}
G_\Lambda\bigl(N_k^{(L)},\delta\bigr)+B_k\bigl(N_k^{(L)}\bigr)\le \varepsilon_r/8,
\end{equation}
so
\begin{equation}
\mathrm{UCB}_{k,r}-\mathrm{LCB}_{k,r}
=
2\Bigl(G_\Lambda\bigl(N_k^{(L)},\delta\bigr)+B_k\bigl(N_k^{(L)}\bigr)\Bigr)
\le \varepsilon_r/4.
\end{equation}
If the chosen fidelity is high, then
\begin{equation}
G_\Lambda\bigl(N_k^{(H)},\delta\bigr)\le \varepsilon_r/8,
\end{equation}
hence
\begin{equation}
\mathrm{UCB}_{k,r}-\mathrm{LCB}_{k,r}
=
2G_\Lambda\bigl(N_k^{(H)},\delta\bigr)
\le \varepsilon_r/4.
\end{equation}
Coverage follows from Lemma~\ref{lem:ci}.
\end{proof}

\begin{lemma}[The optimal arm survives every completed phase]
\label{lem:opt-survives}
Fix a budget $\Lambda>0$ and suppose that the event $\mathcal{E}_\Lambda$ in Lemma~\ref{lem:ci} holds. If phase $r$ is completed, then $k^\star\in\mathcal{S}_{r+1}$.
\end{lemma}

\begin{proof}[Proof sketch]
By Lemma~\ref{lem:phase-width},
\begin{equation}
\mathrm{UCB}_{k^\star,r}\ge \mu^\star
\qquad\text{and}\qquad
\mathrm{LCB}_{k^\star,r}\le \mu^\star.
\end{equation}
Since $\hat{k}_r$ maximizes $\mathrm{LCB}_{k,r}$ over $k\in\mathcal{S}_r$,
\begin{equation}
\mathrm{LCB}_{\hat{k}_r,r}\ge \mathrm{LCB}_{k^\star,r}.
\end{equation}
Therefore
\begin{equation}
\mathrm{UCB}_{k^\star,r}
\ge
\mathrm{LCB}_{\hat{k}_r,r}-\varepsilon_r/4,
\end{equation}
so the optimal arm is not eliminated.
\end{proof}

\begin{lemma}[Phase elimination]
\label{lem:elim}
Fix a budget $\Lambda>0$ and suppose that the event $\mathcal{E}_\Lambda$ in Lemma~\ref{lem:ci} holds. If phase $r$ is completed and $\Delta_k \ge \varepsilon_r$, then arm $k$ is eliminated by the end of phase $r$.
\end{lemma}

\begin{proof}[Proof sketch]
By Lemma~\ref{lem:phase-width},
\begin{equation}
\mathrm{UCB}_{k,r}\le \mu_k^{(H)}+\varepsilon_r/8.
\end{equation}
Also, by Lemma~\ref{lem:opt-survives},
\begin{equation}
\mathrm{LCB}_{\hat{k}_r,r}\ge \mathrm{LCB}_{k^\star,r}\ge \mu^\star-\varepsilon_r/8.
\end{equation}
Hence
\begin{equation}
\mathrm{LCB}_{\hat{k}_r,r}-\varepsilon_r/4
\ge
\mu^\star-\frac{3\varepsilon_r}{8}.
\end{equation}
If $\Delta_k=\mu^\star-\mu_k^{(H)}\ge \varepsilon_r$, then
\begin{equation}
\mathrm{UCB}_{k,r}
\le
\mu_k^{(H)}+\varepsilon_r/8
=
\mu^\star-\Delta_k+\varepsilon_r/8
\le
\mu^\star-\frac{7\varepsilon_r}{8}
<
\mu^\star-\frac{3\varepsilon_r}{8}
\le
\mathrm{LCB}_{\hat{k}_r,r}-\varepsilon_r/4.
\end{equation}
Therefore arm $k$ is eliminated by the end of phase $r$.
\end{proof}

To pass from phase-wise elimination to total exploration cost, we impose a mild regularity condition on the oracle complexity sequence.

\begin{assumption}[Dyadic regularity of oracle costs]
\label{ass:dyadic}
For each suboptimal arm $k\neq k^\star$, there exists a constant $C_{\mathrm{dyad}}>0$ such that
\begin{equation}
\sum_{r\le r_k} \mathsf{c}_k^\star(\varepsilon_r;\Lambda)
\le
C_{\mathrm{dyad}}\, \mathsf{c}_k^\star(\varepsilon_{r_k};\Lambda),
\qquad
r_k := \min\{r:\,\varepsilon_r\le \Delta_k/2\}.
\end{equation}
\end{assumption}

This assumption isolates only the summability step in the phase analysis. It is mild and holds whenever $\mathsf{c}_k^\star(\varepsilon;\Lambda)$ grows at most polynomially as $\varepsilon\downarrow 0$.

\begin{lemma}[Single-phase additional cost upper bound]
\label{lem:phase-cost}
Fix a completed phase $r\le R_\Lambda$ and an arm $k\in\mathcal{S}_r$. Then
\begin{equation}
\Delta\Lambda_{k,r}
\le
\mathsf{c}_k^\star(\varepsilon_r;\Lambda).
\end{equation}
\end{lemma}

\begin{proof}[Proof sketch]
If phase $r$ selects low fidelity for arm $k$, then the algorithm continues querying low fidelity until
\begin{equation}
G_\Lambda\bigl(N_k^{(L)},\delta\bigr)+B_k\bigl(N_k^{(L)}\bigr)\le \varepsilon_r/8.
\end{equation}
Hence the additional low-fidelity cost incurred during phase $r$ is at most the corresponding from-scratch certification cost $\mathsf{c}_k^{(L)}(\varepsilon_r;\Lambda)$. If phase $r$ selects high fidelity, the same argument gives an upper bound by $\mathsf{c}^{(H)}(\varepsilon_r;\Lambda)$. Since phase $r$ chooses the cheaper of the two fidelities at resolution $\varepsilon_r$, the additional phase-$r$ cost is at most
\begin{equation}
\mathsf{c}_k^\star(\varepsilon_r;\Lambda).
\end{equation}
\end{proof}

\begin{proposition}[Oracle elimination cost]
\label{prop:cost}
Fix a budget $\Lambda>0$, and let
\begin{equation}
r_k := \min\{r:\,\varepsilon_r\le \Delta_k/2\}.
\end{equation}
Suppose that the event $\mathcal{E}_\Lambda$ holds and that Assumption~\ref{ass:dyadic} is satisfied. Then any suboptimal arm $k\neq k^\star$ survives for at most the first $r_k$ completed phases, and its total additional phase-based exploration cost before elimination satisfies
\begin{equation}
\sum_{r\le \min\{r_k,R_\Lambda\}} \Delta\Lambda_{k,r}
\le
\sum_{r\le r_k} \mathsf{c}_k^\star(\varepsilon_r;\Lambda)
\le
C\, \mathsf{c}_k^\star(\Delta_k/4;\Lambda)
\end{equation}
for some absolute constant $C>0$.
\end{proposition}

\begin{proof}[Proof sketch]
By Lemma~\ref{lem:elim}, if a completed phase $r$ satisfies $r\ge r_k$, then arm $k$ is eliminated by the end of phase $r$. Therefore arm $k$ can only incur phase-based exploration cost while active in completed phases $1,\dots,r_k$. Summing the phase-wise additional costs and invoking Lemma~\ref{lem:phase-cost} gives
\begin{equation}
\sum_{r\le \min\{r_k,R_\Lambda\}} \Delta\Lambda_{k,r}
\le
\sum_{r\le r_k}\mathsf{c}_k^\star(\varepsilon_r;\Lambda).
\end{equation}
Applying Assumption~\ref{ass:dyadic} and using $\Delta_k/4<\varepsilon_{r_k}\le \Delta_k/2$ yields
\begin{equation}
\sum_{r\le r_k}\mathsf{c}_k^\star(\varepsilon_r;\Lambda)
\le
C_{\mathrm{dyad}}\,\mathsf{c}_k^\star(\varepsilon_{r_k};\Lambda)
\le
C\,\mathsf{c}_k^\star(\Delta_k/4;\Lambda)
\end{equation}
for some absolute constant $C>0$.
\end{proof}

Let $I_t$ denote the arm selected at round $t$, let $m_t\in\{L,H\}$ denote the fidelity selected at round $t$, and define the incurred cost at round $t$ by
\begin{equation}
\lambda_t :=
\begin{cases}
\lambda^{(L)}, & \text{if } m_t=L,\\
\lambda^{(H)}, & \text{if } m_t=H.
\end{cases}
\end{equation}
We define the cost-weighted pseudo-regret as
\begin{equation}
R(\Lambda)
:=
\sum_{t:\,\sum_{s=1}^t \lambda_s \le \Lambda}
\lambda_t \bigl(\mu^\star-\mu_{I_t}^{(H)}\bigr).
\end{equation}

The next theorem is the main result of this section. It shows that the regret is controlled by the arm gaps together with the minimum cost required to certify suboptimality.

\begin{theorem}[Oracle regret under plug-in selected-average envelopes]
\label{thm:main}
Fix a budget $\Lambda>0$ and let $T_\Lambda=\lceil \Lambda/\lambda^{(L)}\rceil$. Under Assumptions~\ref{ass:noise}, \ref{ass:plugin}, and \ref{ass:dyadic}, Algorithm~\ref{alg:rdfe} satisfies, with probability at least $1-\delta$,
\begin{equation}
R(\Lambda)
\le
C_1 \sum_{k\neq k^\star} \Delta_k\, \mathsf{c}_k^\star(\Delta_k/4;\Lambda)
+
(\lambda^{(L)}+\lambda^{(H)})\sum_{k\neq k^\star}\Delta_k
\end{equation}
for some absolute constant $C_1>0$.
\end{theorem}

\begin{proof}[Proof sketch]
For each suboptimal arm $k\neq k^\star$, its regret contribution is at most $\Delta_k$ times the total cost incurred on that arm before elimination. The phase-based part of that cost is controlled by Proposition~\ref{prop:cost}, which yields
\begin{equation}
R_k^{\mathrm{phase}}
\le
C\, \Delta_k\, \mathsf{c}_k^\star(\Delta_k/4;\Lambda).
\end{equation}
In addition, the warm start incurs one low-fidelity query and one high-fidelity query on every arm, so the warm-start regret contribution is at most
\begin{equation}
(\lambda^{(L)}+\lambda^{(H)})\sum_{k\neq k^\star}\Delta_k.
\end{equation}
Summing over all suboptimal arms proves the theorem.
\end{proof}

The theorem isolates the right benchmark quantity for the present oracle-envelope setting. The difficulty of learning arm $k$ is not governed by a static fidelity gap, but by the minimum cost required to certify suboptimality at resolution $\Delta_k$.

Under the standard normalization $\mu_k^{(H)}\in[0,1]$, one has $\Delta_k\le 1$, and the warm-start term simplifies to
\begin{equation}
(\lambda^{(L)}+\lambda^{(H)})\sum_{k\neq k^\star}\Delta_k
\le
K(\lambda^{(L)}+\lambda^{(H)}).
\end{equation}

A standard truncation argument now yields a generic gap-independent upper bound.

\begin{corollary}[Generic gap-independent bound]
\label{cor:gap}
Under the assumptions of Theorem~\ref{thm:main},
\begin{equation}
R(\Lambda)
\le
C
\inf_{\varepsilon\in(0,1]}
\left\{
K\sup_{x\ge \varepsilon} x\, \mathsf{c}^\star(x;\Lambda)
+
\Lambda \varepsilon
\right\}
+
(\lambda^{(L)}+\lambda^{(H)})\sum_{k\neq k^\star}\Delta_k,
\end{equation}
where
\begin{equation}
\mathsf{c}^\star(x;\Lambda)
:=
\sup_{k\neq k^\star} \mathsf{c}_k^\star(x;\Lambda).
\end{equation}
\end{corollary}

\begin{proof}[Proof sketch]
Fix $\varepsilon\in(0,1]$ and partition the suboptimal arms into
\begin{equation}
\mathcal{A}_\varepsilon := \{k\neq k^\star:\Delta_k\ge \varepsilon\},
\qquad
\mathcal{B}_\varepsilon := \{k\neq k^\star:\Delta_k<\varepsilon\}.
\end{equation}
For the first group,
\begin{equation}
\sum_{k\in\mathcal{A}_\varepsilon}
\Delta_k\, \mathsf{c}_k^\star(\Delta_k/4;\Lambda)
\le
K\sup_{x\ge \varepsilon} x\, \mathsf{c}^\star(x;\Lambda).
\end{equation}
For the second group, each selected arm contributes at most $\varepsilon$ regret per unit cost, so the total contribution is at most $\Lambda\varepsilon$. Combining these bounds with Theorem~\ref{thm:main} and optimizing over $\varepsilon$ yields the result.
\end{proof}

The main message is simple: once the low-fidelity source is modeled through a plug-in selected-average envelope induced by a cumulative mismatch certificate, fidelity selection becomes a resolution-dependent decision problem, and the regret is naturally governed by the oracle complexity $\mathsf{c}_k^\star(\varepsilon;\Lambda)$.
